Statistical Depth for Ranking and Characterizing Transformer-Based Text Embeddings

The popularity of transformer-based text embeddings calls for better statistical tools for measuring distributions of such embeddings. One such tool would be a method for ranking texts within a corpus by centrality, i.e. assigning each text a number signifying how representative that text is of the corpus as a whole. However, an intrinsic center-outward ordering of high-dimensional text representations is not trivial. A statistical depth is a function for ranking k-dimensional objects by measuring centrality with respect to some observed k-dimensional distribution. We adopt a statistical depth to measure distributions of transformer-based text embeddings, transformer-based text embedding (TTE) depth, and introduce the practical use of this depth for both modeling and distributional inference in NLP pipelines. We first define TTE depth and an associated rank sum test for determining whether two corpora differ significantly in embedding space. We then use TTE depth for the task of in-context learning prompt selection, showing that this approach reliably improves performance over statistical baseline approaches across six text classification tasks. Finally, we use TTE depth and the associated rank sum test to characterize the distributions of synthesized and human-generated corpora, showing that five recent synthetic data augmentation processes cause a measurable distributional shift away from associated human-generated text.

==> sections/depth.tex <==
\section{Transformer-based Text Embedding Depth}
\label{sec:depth}

Angular distance properties of text embeddings, such as high cosine similarity between embeddings of two similar texts, are often sought as a desired property of such embeddings \cite{reimers-2019-sentence-bert}. As such, we utilize an angular distance-based depth for our investigation. A class of angular distance-based depths for directional data was first introduced by \cite{pandolfo2018distance}, and later used by \cite{pandolfo2021depth} for classification of directional data. Leaning on two depth definitions as introduced there we define a depth for transformer-based text embeddings, TTE depth.

\textbf{TTE depth:} Consider a corpus of embedded texts $\mathcal{F}$ derived from the theoretical set of all possible such documents $S$, each embedded by some text embedding model $M: S \rightarrow \mathbb{R}^k$ which embeds texts into vectors of length $k$. Given a bounded distance $\delta(\cdot, \cdot): S \times S \rightarrow \mathbb{R}$, the TTE depth of an embedded text $x \in \mathcal{F}$ with respect to $\mathcal{F}$ is defined as 

\begin{equation}
\label{eq:depth}
    D_\delta(x,\mathcal{F}) := 2 - E_\mathcal{F}[\delta(x,H)]
\end{equation}


Where $E_\mathcal{F}$ is the expectation under the assumption that $H$ has distribution $\mathcal{F}$, i.e. $H$ represents the realized values of corpus $\mathcal{F}$. Note also that while $M$ could be \textit{any} text embedding model, in this work we specifically investigate transformer-based embedding methods.

TTE depth can be used in conjunction with two bounded distance functions.

The \textbf{cosine distance} $cos(\cdot,\cdot)$ between two embedded text documents $x, y \in \mathcal{F}$ is well explored as a tool for examining pairwise relationships between transformer-based text embeddings \cite{sunilkumar2019survey}. It is defined as

\begin{equation}
    cos(x,y) := 1 - \frac{x \cdot y}{\|x\| \|y\|}
\end{equation}

For any two embedded texts $x, y \in \mathcal{F}$, the \textbf{chord distance} $ch(\cdot,\cdot)$ between the two is defined as

\begin{equation}
    ch(x,y) := \sqrt{2(1-x'y)}
\end{equation}

While we primarily investigate TTE depth using cosine distance, either cosine distance and chord distance can be used for calculating TTE depth. Importantly, as shown by \cite{pandolfo2018distance}, using either distance function means TTE depth will hold the following properties.

%\textit{Rotation invariance:} Since $D_\delta(x,\mathcal{F}) = D_\delta(Ox,O\mathcal{F})$ for any $k \times k$ orthogonal matrix $O$, TTE depth is rotation invariant.

\textit{Maximality at center:} If $\mathcal{F}$ has center at $x_0$, TTE depth is maximal at center since $max_{x \in \mathcal{F}} D_\delta(x, \mathcal{F}) = D_\delta(x_0, \mathcal{F})$.

\textit{Monotonicity from the deepest point:} $D_\delta$ decreases along any shortest path from $x_0$ to its antipodal (diametrically opposite) point, call it $-x_0$.

These two properties allow TTE depth to produce a well-defined median (i.e. text with highest TTE depth) at the center of the distribution of text embeddings, as well as a gradual center-outward ranking of all text embeddings within a corpus.

\textbf{Wilcoxon Rank Sum Test:} As TTE depth gives an ordering to a corpus of text embeddings, we can use an existing rank sum test for determining whether the embeddings of two corpora differ significantly. Existing applications of depth utilize the Wilcoxon rank sum test generalized to multivariate data through the order induced by a depth function \cite{lopez2009concept, liu1993quality}; we follow these works in our definitions. 

Suppose we have two corpora, and the distributions of the embeddings in $\mathbb{R}^k$ of texts within these corpora are given by $F$ and $G$. We wish to determine whether it is unlikely that $G$ follows the same distribution as $F$. For a given text embedding $y \in G$, we first define $R(y,F)$ as the fraction of the $F$ population which is "less central" to $F$ than the embedding $y$. Given that $X \sim F$,

\begin{equation}
    R(y,F) = P_F\{D_\delta(X,F) \le D_\delta(y,F) \}
\end{equation}

This roughly measures how well a given text embedding $y \in G$ fits in the distribution of text embeddings in $F$. For example, if $R(y,F)$ is low, then a large portion of the text embeddings in $X$ are more central to $F$ than $y$, indicating that $y$ is an outlier with respect to $F$. Next we use $R(y,F)$ to define the $Q$ parameter to gauge the overall "outlyingness" of the $G$ population with respect to the given $F$ population. Given that $X \sim F$ and $Y \sim G$,

\begin{equation}
    Q(F,G) = P\{D_\delta(X,F) \le D_\delta(Y,F)\}
\end{equation}

Since $R(y,F)$ is the fraction of the $F$ corpus which is "less central" to $F$ than the value $y$, $Q(F,G)$ is the average of such fractions over all $y$'s from the $G$ corpus. This means that $Q$ allows us to characterize and quantify how two corpus distributions differ in embedding space. When $Q < \frac{1}{2}$, it means on average more than 50\% of the $F$ corpus is deeper than text embeddings $Y$ from $G$, indicating $Y$ is more outlying than $X$ with respect to $F$, hence an inconsistency between $F$ and $G$. 

We use the $Q$ parameter to test whether $F$ and $G$ are likely to have come from the same distribution. \cite{liu1993quality} propose a Wilcoxon rank sum test for the hypotheses $H_O: F = G$ versus $H_a: Q < \frac{1}{2}$. Let $X = \{x_1, x_2, ..., x_m \}$ and $Y = \{y_1, y_2, ..., y_n\}$ be samples of text embeddings from $F$ and $G$, respectively. A sample estimate of $Q$ is $Q(F_m, G_n) = \frac{1}{n} \sum\limits_{i=1}^{n} R(y_i,F_m)$, where $R(y_i,F_m)$ is the proportion of $x_j$'s having $D_\delta(x_j,F_m) \le D_\delta(y_i,F_m)$. In other words, $Q(F_m, G_n)$ is the average of the ranks of $y_i$'s in the combined sample $X \cup Y$. If this sample estimate is low, we consider the likelihood that the samples $X$ and $Y$ come from the same distribution of text embeddings to be low, and say that it is instead likely that the distributions of $F$ and $G$ differ significantly. As empirically shown in \cite{liu1993quality}, the null distribution of $W = [Q(F_m, G_n) - Q(F,G)]$ is approximated by $\mathcal{N}(0, \frac{\frac{1}{m} + \frac{1}{n}}{12})$, and a $Z$ test can be used from there. We give a detailed example of how to interpret the $Q$ parameter and the Wilcoxon rank sum test in Section \ref{sec:results:synth}.

% As an example of how to interpret the results of the Wilcoxon rank sum test, consider the following toy example. Suppose we have collected some number of post responses from an online message board, with half the responses (bot corpus) being produced by a bot and half being produced by human users (human corpus). To test whether responses in the bot corpus differ significantly from responses in the human corpus, we can embed each response in each corpus using a transformer-based text embedding model such as S-BERT. We run a Wilcoxon rank sum test based on the ordering induced by the TTE depth of the human and bot corpora and obtain a test statistic $W = -1.01$ and a $p$-value of $0.3131$. Based on this test, we can say there is insufficient evidence to show that the bot corpus differs significantly in embedding space from the human corpus.


==> sections/old_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

To investigate the usefulness of directional depth in a variety of scenarios involving transformer-based text embeddings, we perform experiments across three different task formulations. While these tasks differ in scope and purpose, we show that each benefits from the corpus-level center-outward ranking of text documents provided by directional depth. In each scenario, we embed the relevant corpus of texts using S-BERT, a popular transformer-based text embedding model \cite{}. \textcolor{red}{explain why using S-BERT alone is good enough, otherwise we'll want to test a couple other embedding models.} Unless otherwise stated, we report directional depth statistics using both the chord distance and the cosine distance. 

\subsection{Ranking of Few-Shot Exemplars for In-Context Learning}
\label{sec:experiments:icl}

In-context learning (ICL) is a recent paradigm used for few-shot settings of common NLP tasks. In text classification it involves prompting a pre-trained language model (PLM) to assign a label to an unseen input after being seeing several exemplars \cite{}. While ICL has achieved competitive results across a variety of text classification benchmarks in the few-shot setting, it is also a useful benchmark for complex classification tasks with larger training datasets available \cite{} \textcolor{red}{CAN CITE MYSELF HERE}. As such, recent work has investigated both how ICL works \cite{} and how to select representative exemplars from training datasets of varying sizes \cite{}. We propose the use of directional depth for the selection of representative exemplars for ICL. To do so, we extrinsically evaluate test two depth-based rankings against two baseline rankings across two different text classification tasks. 

\textbf{Random (RAND)} This benchmark ranking simply randomly shuffles the training dataset, after which the first $N$ texts are used as ICL exemplars.

\textbf{Label Distribution Match (LDM)} Another simple benchmark is to ensure that the label distribution of the training dataset is matched by the selected ICL exemplars. For each label occupying $l\%$ of the training data label space, after applying a random shuffle the first $N \cdot l\%$ texts with that label are selected as ICL exemplars. This ranking attempts to ensure that the PLM is able to accurately infer the label distribution of the training data through the ICL exemplars.

\textbf{Depth (DEEP)} The depth ranking simply ranks all embedded texts by their directional depth. Then, the $N$ deepest texts are selected as ICL exemplars.

\textbf{Depth with Label Distribution Match (DLDM)} As a combination of both the depth ranking and the label distribution match, this ranking first ranks all embedded texts by their directional depth. Then, the same selection strategy as the label distribution match ranking is used. Hence, the $N \cdot l\%$ deepest texts for each label are selected as ICL exemplars.

Following \cite{longpre2020effective}, we utilize 6 text classification datasets for testing each ranking method. \textcolor{red}{DESCRIBE EACH TASK}

For each task, we embed each text in the training corpus using S-BERT. Next, we rank each embedded text according to each of the benchmark and depth-based ranking strategies described. The $N$ ICL exemplars given by each ranking strategy are then used in the ICL prompt. We use this prompt to query ChatGPT \cite{}, a popular PLM which has been shown to offer good performance across several ICL text classification tasks \cite{}, to label each test sample. After post-processing, results are recorded for each ranking strategy across different values of $N$.

% We test each ranking method across two different text classification tasks. The first task is the well-known \textit{IMDB review sentiment classification} benchmark \cite{}. As ICL with a premier PLM across a large test dataset can be prohibitively expensive, we randomly sample 1,000 test reviews for our evaluation. The second task is a low-resource text multiclass classification task. As ICL is a few-shot ... 

\subsection{Semantic Textual Similarity}
\label{sec:experiments:sts}

A common task involving statistical depths is the classification of unseen observations according to their  centers of distributions

\subsection{Investigation of Augmented Corpora}

Next, we use of depth as a corpora comparison tool to investigate the distribution shift in PLM and human-generated data augmentation strategies. Specifically, we compare two popular task-agnostic data augmentation strategies with a simple human-generated data augmentation using directional depth for transformer-based embeddings. As in the recent investigation of task-agnostic data augmentation strategies in cite{}, we compare  Easy Data Augmentation (EDA) \cite{} and Back-Translation (BT) \cite{}. % https://arxiv.org/pdf/2010.01764.pdf, https://arxiv.org/pdf/1901.11196.pdf, https://arxiv.org/abs/1511.06709

To validate the use of directional depth for transformer-based embeddings as a corpora comparison tool, we investigate its use alongside other common corpora comparison tools \cite{}. % https://github.com/HLasse/TextDescriptives

\label{sec:experiments:augmented}
